SoK: Lending Pools in Decentralized Finance

Lending pools are decentralized applications which allow mutually untrusted users to lend and borrow crypto-assets. These applications feature complex, highly parametric incentive mechanisms to equilibrate the loan market. This complexity makes the behaviour of lending pools difficult to understand and to predict: indeed, ineffective incentives and attacks could potentially lead to emergent unwanted behaviours. Reasoning about lending pools is made even harder by the lack of executable models of their behaviour: to precisely understand how users interact with lending pools, eventually one has to inspect their implementations, where the incentive mechanisms are intertwined with low-level implementation details. Further, the variety of existing implementations makes it difficult to distill the common aspects of lending pools. We systematize the existing knowledge about lending pools, leveraging a new formal model of interactions with users, which reflects the archetypal features of mainstream implementations. This enables us to prove some general properties of lending pools, such as the correct handling of funds, and to precisely describe vulnerabilities and attacks. We also discuss the role of lending pools in the broader context of decentralized finance.

==> basic_amm.tex <==
\section{Automatic Market Makers} \label{section:amm}
\jamesnote{Use partial maps.}
A constant function automatic market maker (AMM) is a DeFi archetype which allows a user to swap units of a token type $\tokT[0]$ for units of another type $\tokT[1]$ and back without the need to find a counter-party seeking a matching swap. Instead, an AMM provides token pair funds, which a user can interact with. There are two types of interactions with an AMM: The \emph{liquidity provider} provides funds to a swap pair $\tokT, \tokTi$, where $\tokT \neq \tokTi$, and earns a fee on each swap transaction performed. Subsequently, a user can swap units of $\tokT$ for units of $\tokTi$ and vice versa. The exchange rate $\tokTi / \tokT$ is a function of the AMM pair funds, and is therefore effected by each swap transaction. However, given a difference between exchange rates implied by $\exchO$ and an AMM pair, and assuming that a user can freely exchange tokens at rates implied by $\exchO$, there exists an incentive interact with an AMM until they are equal. In the following example, we illustrate how a single AMM pair is initially funded by user $\pmvA$, after which agents $\pmvB$ and $\pmvC$ can execute swaps between token types. We write $\ammRi[0], \ammRi[1]$ to denote funds of each token type in the respective AMM token pair after the execution of each transaction shown row-wise. 

\begin{table}[h!]
\centering
\begin{tabular}{llllll}
Transaction & $\tokBal[\pmvA]$ 
    & $\tokBal[\pmvB]$ & $\tokBal[\pmvC]$ & $\ammRi[0]$ & $\ammRi[1]$ \\ \hline
    & $100:\tokT[0], 100:\tokT[1]$ 
    & $100:\tokT[0]$ 
    & $50:\tokT[1]$ &  \\ \hline
1. $\pmvA$ dep. $\tokT[0], \tokT[1]$ 
    & $100:\tokT[0|1]$ 
    & $100:\tokT[0]$ \;
    & $50:\tokT[1]$ 
    & $100:\tokT[0]$ & $100:\tokT[1]$ \\ \hline
2. $\pmvB$ swaps $\tokT[0]$ for $\tokT[1]$ 
    & $100:\tokT$ 
    & $50:\tokT[1]$ 
    & $50:\tokT[1]$ 
    & $200:\tokT[0]$ & $50:\tokT[1]$ \\ \hline  
3.  $\pmvA$ redeems $\tokT$ 
    & $20:\tokT[0], 5:\tokT[1], 90:\tokT[0|1]$ 
    & $50:\tokT[1]$ 
    & $50:\tokT[1]$ 
    & $180:\tokT[0]$ & $45:\tokT[1]$ \\ \hline
4.  $\pmvC$ swaps $\tokT[1]$ for $\tokT[0]$
    & $20:\tokT[0], 5:\tokT[1], 90:\tokT[0|1]$ \; 
    & $50:\tokT[1]$ 
    & $\frac{1800}{19}:\tokT[0] $ 
    & $\frac{1620}{19}:\tokT[0]$ & $95:\tokT[1]$\\ \hline
\end{tabular}
\end{table}

In transaction 1, user $\pmvA$ deposits equal amounts of $\tokT[0]$ and $\tokT[1]$ into the AMM pair. $\pmvA$ receives $100:\tokT$ minted by specifically for token pair $(\tokT[0] ,\tokT[1])$: Each unit of $\tokT$ represents a claim to \emph{both} token reserves $\ammR[0]$ and $\ammR[1]$. The claim of a single minted token unit is proportional to the total minted supply for the specific token pair. In transaction two, user $\pmvB$ swaps $100:\tokT[0]$ for $50:\tokT[1]$. Note the exchange rate is entirely a function of $\ammR[0],\ammR[1]$, such that the product $\ammR[0] \cdot \ammR[1] = \ammRi[0] \cdot \ammRi[1]$ is preserved with each swap transaction. In transaction 2, user $\pmvA$ redeems $10:\tokT$, reducing the funds in the AMM token pair. In the final transaction, user $\pmvC$ performs a swap in the opposite direction than user $\pmvB$ by swapping $50:\tokT[1]$ for units of $\tokT[0]$. We note that user $\pmvC$ only receives $\frac{1800}{19} \approx 94.7$ of $\tokT[0]$, which is less than user $\pmvB$'s original balance of $100:\tokT[0]$. This is due to the reduced reserves caused by the preceding redeem transaction. 
\jamesnote{AL: circularity of tokens, constrain against?}
\jamesnote{Constrain against trading minted tokens?}
\paragraph{Configuration with Automatic Market Makers:} We write $\AmmS$ to denote the state of a single AMM instance in the configuration
\[
\confDep{\pmvA[1]}{\tokBal[1]} \mid \cdots \mid \confDep{\pmvA[n]}{\tokBal[n]}
\mid \AmmS \mid \exchO \mid \br
\]
Here, $\AmmS$ is the record $\left\{ \ammF:\ammFfun, \ammM:\ammMfun \right\}$ where $\ammFfun$ represents a map from token pairs ($\TokU \times \TokU$) to a token pair balance ($\Nat \times \Nat$), and $\ammMfun$ a map from token pairs to the corresponding minted token type and minted units ($\TokU \times \Nat$). 

\begin{table}[h!]
\centering
\begin{tabular}{ll}
    $\AmmS.\ammF = \ammFfun 
        \in \TokU \times \TokU \rightarrow \Nat \times \Nat$ & Token pair funds \\
    $\AmmS.\ammM = \ammMfun 
        \in \TokU \times \TokU \rightarrow \TokU \times \Nat$ & Minted tokens \\
\end{tabular}
\caption{Notation: Automatic Market Maker (AMM)}
\end{table}
\noindent
We extend our previous notion of updating a token balance (eq. \ref{eq: balance update}) to an AMM \emph{token pair} balance $\ammFfun$, where each update occurs for a \emph{pair} of token types. We write $\ammR, \ammRi$ to denote the funds in an AMM pair $(\tokT,\tokTi)$.
\begin{equation} \label{eq: pair balance update}
\begin{array}{l}
    \sigma_{p} \circ (\valV, \valVi):(\tokT, \tokTi) = \begin{cases}
      \sigma_{p}\setenum{\bind{(\tokT, \tokTi)}{(\ammR\;\circ\;\valV, \;\ammRi\;\circ\;\valVi)}}
      & \circled{1}\; \mathit{if} \; \left\{ \tokT, \tokTi \right\} \subseteq  \mathit{pairs}(\AmmS) \\
      \sigma_{p} \setenum{\bind{(\tokT,\tokTi)}{(\valV, \valVi)}}
      & \circled{2}\; \mathit{if} \; \left\{ \tokT, \tokTi \right\} \not\subseteq  \deposited(\AmmS) \\
    \end{cases} \\[1.3em]
    \ammR, \ammRi = \AmmS.\ammF(\tokT, \tokTi) \qquad 
    \mathit{pairs}(\AmmS) = \dom(\AmmS.\ammM) \\
    \deposited(\AmmS) = \left\{ (\tokTi, \tokTii) \mid (\tokTi, \tokTii) \in \mathit{pairs}(\AmmS) \vee (\tokTii, \tokTi) \in \mathit{pairs}(\AmmS) \right\} 
\end{array} 
\end{equation}
Note that token type pairs in $\dom(\ammFfun)$ are \emph{ordered}. The update function of $\ammFfun$ ensures that a previously deposited token pair $\tokT, \tokTi$ cannot be added in reverse order (\circled{2} in eq. \ref{eq: pair balance update}). This enforces the the initial ordering of a token pair in $\dom(\AmmS.\ammF)$ for all subsequent states $\confGi$ reachable from $\confG$. 

\paragraph{AMM-Initial:} We write that a configuration $\confDep{\pmvA[1]}{\tokBal[1]} \mid \cdots \mid \confDep{\pmvA[n]}{\tokBal[n]} \mid \AmmS \mid \exchO \mid \br$ is AMM-initial if domains of $\AmmS.\ammF$, $\AmmS.\ammM$ are both $\emptyset \times \emptyset$.

\paragraph{AMM Deposit:} A \emph{liquidity provider} is a user who deposits units of both token types of a AMM token pair $\tokT[0], \tokT[1]$. Funds of both types are deposited to the AMM \circled{5},\circled{6}, such that the unit ratio between the deposited tokens $\valV[0]/\valV[1]$ is equal to the unit ratio of the token pair funds $\ammR[0]/\ammR[1]$ before and after the deposit \circled{1}. For the initial deposit to an AMM token pair $\tokT[0],\tokT[1]$, any ratio of deposited units is permitted \circled{1}. The deposit of a single token type, however, is not permitted: Each pair token pair initially requires funds in both types to enable subsequent swap transactions. Furthermore, minted token units represent equal claims on deposits of \emph{both} token types, which would be contradicted by the minting of tokens for the deposit of a single token type only. 
% \begin{equation} \label{eq: amm deposit transaction}
% \irule
% {
% \begin{array}{l}
%     \begin{array}{ll}
%         \circled{1}\;(\tokBal[\pmvA](\tokT[0]),\tokBal[\pmvA](\tokT[1])) \geq (\valV[0], \valV[1]) > (0,0) 
%             & \circled{2}\; \tokT[0] \neq \tokT[1] \\
%         \circled{3}\; \valVi := \frac{\valV[0]}{\fst(\ER[\AmmS]{\tokT[0],\tokT[1]})} 
%             \quad \valVii := \frac{\valV[1]}{\snd(\ER[\AmmS]{\tokT[0],\tokT[1]})} \quad \;
%             & \\
%         \circled{4}\; \tokBali[\pmvA] := \tokBal[\pmvA] - \valV[0]:\tokT[0] -\valV[1]:\tokT[1] + \valV:\tokT \quad\;
%             & \valV = \min(\valVi,\valVii) \\
%         \circled{5}\; \ammFfuni := \AmmS.\ammF + (\valV[0],\valV[1]):(\tokT[0], \tokT[1])
%             & \\
%     \end{array} \\
%     \begin{array}{l}
%         \circled{6}\; \ammMfuni := \begin{cases}
%             \AmmS.\ammM\setenum{\bind{(\tokT[0], \tokT[1])}{(\tokT,\valV)}} 
%                 & \mathit{if} \; (\tokT[0], \tokT[1])  \nsubseteq  \deposited(\AmmS.\ammM) \quad  \mathit{fresh}\;\tokT \\
%             \AmmS.\ammM\setenum{\bind{(\tokT[0], \tokT[1])}{(\tokT,\valViii+\valV)}}
%                 & \mathit{if} \;  (\tokT, \valViii) = \AmmS.\ammM(\tokT[0],\tokT[1])
%         \end{cases}
%     \end{array}
% \end{array}
% }{
%     \confDep{\pmvA}{\tokBal[\pmvA]} \mid
%     \AmmS \mid
%     \confG[e]
%     \xrightarrow{\actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}}
%     \confDep{\pmvA}{\tokBali[\pmvA]} \mid 
%     \AmmS \setenum{ \ammF = \ammFfuni, \ammM = \ammMfuni} \mid
%     \confG[e]
% }
% \end{equation}
\begin{equation} \label{eq: amm deposit transaction}
\irule
{
\begin{array}{l}
    \begin{array}{l}
        \circled{1}\; \valV[1] = \begin{cases}
            \frac{\ammR[1]}{\ammR[0]} \cdot \valV[0]  
                & \mathit{if} \; \; (\ammR[0],\ammR[1])=\AmmS.\ammF(\tokT[0], \tokT[1]) > (0,0)  \\
            \valV[1]
                & \mathit{otherwise} 
        \end{cases}
    \end{array} \\
    \begin{array}{ll}
        \circled{2}\;(\tokBal[\pmvA](\tokT[0]),\tokBal[\pmvA](\tokT[1])) \geq (\valV[0], \valV[1]) > (0,0) 
            & \circled{3}\; \tokT[0] \neq \tokT[1] \\
        \circled{4}\; \valV := \frac{\valV[0]}{\fst(\ER[\AmmS]{\tokT[0],\tokT[1]})} 
            = \frac{\valV[1]}{\snd(\ER[\AmmS]{\tokT[0],\tokT[1]})} \quad \;
            & \\
        \circled{5}\; \tokBali[\pmvA] := \tokBal[\pmvA] - \valV[0]:\tokT[0] -\valV[1]:\tokT[1] + \valV:\tokT \quad\;
            & \circled{6}\; \ammFfuni := \AmmS.\ammF + (\valV[0],\valV[1]):(\tokT[0], \tokT[1]) \\
    \end{array} \\
    \begin{array}{l}
        \circled{7}\; \ammMfuni := \begin{cases}
            \AmmS.\ammM\setenum{\bind{(\tokT[0], \tokT[1])}{(\tokT,\valV)}} 
                & \mathit{if} \; (\tokT[0], \tokT[1])  \nsubseteq  \deposited(\AmmS.\ammM) \quad  \mathit{fresh}\;\tokT \\
            \AmmS.\ammM\setenum{\bind{(\tokT[0], \tokT[1])}{(\tokT,\valViii+\valV)}}
                & \mathit{if} \;  (\tokT, \valViii) = \AmmS.\ammM(\tokT[0],\tokT[1])
        \end{cases}
    \end{array}
\end{array}
}{
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid
    \AmmS \mid
    \confG[e]
    \xrightarrow{\actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}}
    \confDep{\pmvA}{\tokBali[\pmvA]} \mid 
    \AmmS \setenum{ \ammF = \ammFfuni, \ammM = \ammMfuni} \mid
    \confG[e]
}
\end{equation}
\jamesnote{WIP: Note ER may be inconsistent with pr.}
The AMM mints units of a token type specific to each deposited token pair $\circled{4},\circled{7}$. The exchange rate of the minted token to deposited token types is given by
\begin{equation} \label{eq: amm exchange rate}
\begin{array}{l}
    \ER[\AmmS]{\tokT[0],\tokT[1]} = \begin{cases}
      \dfrac
      {(\ammR[0],\ammR[1])}
      {\snd(\AmmS.\ammM(\tokT[0], \tokT[1]))} 
      & \mathit{if} \; 
        \begin{array}{l}
            \left\{ \tokT[0], \tokT[1] \right\} \in \dom(\AmmS.\ammM) \\
            (\ammR[0],\ammR[1]) = \AmmS.\ammF(\tokT[0], \tokT[1])
        \end{array} \\
      1
      & \textit{otherwise}
    \end{cases} 
\end{array}
\end{equation}
A \emph{liquidity provider} is incentivized to provide deposits to a given AMM pair as it will earn \emph{fees} for each subsequent \emph{swap} transaction executed on the token pair.

\jamesnote{AmmSwap, not Swap.}

\paragraph{AMM Swap:} A user swaps from $\tokT$ to $\tokTi$ if it transfers units of $\tokT$ to an AMM pair in return for units of $\tokTi$, given a positive AMM pair balance \circled{1} and a sufficient balance of $\pmvA$. We denote $\actAmmSwap{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$ as a swap by $\pmvA$, who \emph{transfers} $\valV[0]:\tokT[0]$ and \emph{receives} $\valV[1]:\tokT[1]$ for $\valV[0] < 0$ \circled{2}. We denote a swap in the opposite direction for $\valV[0] > 0$ and $\valV[1] < 0$ with the same transaction rule shown below.

\jamesnote{Can a user deposit a pair of funds based on a view of the future price. Abstracts away fees on the simplified model.}
\begin{equation} \label{eq: amm swap transaction}
\irule
{
\begin{array}{l}
    \begin{array}{ll}
        \circled{1}\; \ammR[0], \ammR[1] := \AmmS.\ammF(\tokT[0],\tokT[1]) > (0,0) 
            &  \\
    \end{array} \\
    \begin{array}{l}
        \circled{2}\; \tokBal[\pmvA](\tokT[0]) \geq -\valV[0] > 0 \;\;
            \vee \;\; \tokBal[\pmvA](\tokT[1]) \geq -\valV[1] > 0 \\
    \end{array} \\
    \begin{array}{l}
        \circled{3}\; \valVi[0], \valVi[1], \ammRi[0], \ammRi[1] := \begin{cases}
            (1-c_{fee}) \cdot \valV[0], \valV[1], \ammR[0] + c_{fee}\cdot\valV[0] , \ammR[1] 
                & \mathit{if} \; \; \valV[0] < 0  \\
            \valV[0], (1-c_{fee}) \cdot \valV[1], \ammR[0], \ammR[1] + c_{fee}\cdot\valV[1]
                & \mathit{otherwise} 
        \end{cases} \\
    \end{array} \\
    \begin{array}{ll}
        \circled{4}\; (\ammRi[0] - \valVi[0])(\ammRi[1] - \valVi[1]) = \ammRi[0]\cdot \ammRi[1] 
            \;\quad\; & (\valVi[0],\valVi[1]) 
                = (\frac{\ammRi[0]}{\valVi[1]-\ammRi[1]} \cdot \valVi[1]), 
                    (\frac{\ammRi[1]}{\valVi[0]-\ammRi[0]} \cdot \valVi[0]) \\
    \end{array}\\
   \begin{array}{l}
    \circled{5}\; \valVii[0], \valVii[1] := \begin{cases}
        \valV[0], \valVi[1] 
            & \mathit{if} \; \; \valV[0] < 0  \\
        \valVi[0], \valV[1]
            & \mathit{otherwise} 
    \end{cases} \\
    \end{array} \\ 
    \begin{array} {ll}
        \circled{6}\; \tokBali[\pmvA] := \tokBal[\pmvA] + \valVii[0]:\tokT[0] + \valVii[1]:\tokT[1] \;\quad\;
            & \circled{7}\; \ammFfuni := \AmmS.\ammF - (\valVii[0], \valVii[1]):(\tokT[0], \tokT[1]) \\
    \end{array}
\end{array}
}
{\begin{array}{l}
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid \AmmS \mid 
    \confG[e]
    \xrightarrow{\actAmmSwap{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}}
    \confDep{\pmvA}{\tokBali[\pmvA]} \mid
    \AmmS \setenum{\ammF = \ammFfuni} \mid
    \confG[e] 
 \end{array}}
\end{equation}
\jamesnote{AL: Why swap does not involve minted tokens, does it not affected value of minted token?}
Each swap transaction directs a fraction of the \emph{transferred} token to the respective fund of an AMM pair $\tokT[0],\tokT[1]$ \circled{3}, which can later be claimed by holders of the minted pair token $\AmmS.\ammM(\tokT[0],\tokT[1])$ with a redeem transaction. A swap transaction implies an exchange rate between the token pair types, which is function of the token pair balance ($\ammR[0], \ammR[1] = \AmmS.\ammF(\tokT[0],\tokT[1])$) and swapped funds amounts \circled{4}. In particular a swap transaction maintains a constant product of token pair funds, such that $c=\ammR[0]\cdot\ammR[1] =\ammRi[0]\cdot\ammRi[1]$ for $\confG \xrightarrow{\ammSwapOp} \confGi$. 


\paragraph{AMM Redeem:} A user holding a positive balance of $\tokT = \AmmS.\ammM(\tokT[0],\tokT[1])$ can redeem these tokens in return for units of $\tokT[0], \tokT[1]$ \circled{4}. Here, the redeemable amount of $\tokT[0]$ and $\tokT[1]$ is determined by the exchange rate in eq. \ref{eq: amm exchange rate}: Each unit of minted $\tokT$ is equally redeemable for amounts of each token pair type \circled{2},\circled{3}.
\begin{equation} \label{eq: amm redeem transaction}
    \irule
    {
    \begin{array}{ll}
        \circled{1}\;\tokBal[\pmvA](\tokT) \geq  \valV 
            &  \\
        \circled{2}\; \valVi[0] := \valV \cdot \fst(\ER[\AmmS]{\tokT[0],\tokT[1]})     
            & \fst(\LpS.\lpM(\tokT[0], \tokT[1])) = \tokT \\
        \circled{3}\; \valVi[1] :=  \valV \cdot \snd(\ER[\AmmS]{\tokT[0],\tokT[1]}) 
            & \\      
        \circled{4}\; \tokBali[\pmvA] := \tokBal[\pmvA] + \valVi[0]:\tokT[0] + \valVi[1]:\tokT[1] - \valV:\tokT \quad\;
            & \circled{5}\; \ammFfuni := \AmmS.\ammF - (\valVi[0], \valVi[1]):(\tokT[0], \tokT[1]) \\
        \circled{6}\; \ammMfuni := \AmmS.\ammM\setenum{\bind{\uTok(\tokT)}{(\tokT,\valVii-\valV)}} \;\;
            & (\tokT,\valVi) := \AmmS.\ammM(\tokT[0], \tokT[1]) 
    \end{array}
    }
    {\begin{array}{l}
        \confDep{\pmvA}{\tokBal[\pmvA]} \mid \AmmS \mid 
        \confG[e]
        \xrightarrow{\actRedeem{\pmvA}{\valV:\tokT}}
        \confDep{\pmvA}{\tokBali[\pmvA]} \mid
        \AmmS \setenum{ \ammF = \ammFfuni, \ammM = \ammMfuni} \mid
        \confG[e] 
        \end{array}
    } \\
\end{equation}
% \[
% \begin{array}{l}
%     \minted(\AmmS) = \left\{ \tau \mid \exists (\tokTi, \tokTii) : \fst(\LpS.\lpM(\tokTi, \tokTii)) = \tokT \right\} \\
% \end{array}
% \]
\subsection{AMM Properties}
We now proceed to describe noteworthy properties of automatic market makers as previously defined. For simplicity, we ignore fees in the $\ammSwapOp$ transaction type, such that $C_{fee}=0$ in eq. \ref{eq: amm swap transaction}. 

\paragraph{AMM swap properties:} The swap transaction type is intended for users to swap units of tokens between token types of AMM pairs without a counter-party to execute an opposite, matching swap. Each AMM pair with a positive pair balance maintains a constant product invariant over its pair funds, and allows for a transfer for any finite amount in a swap transaction.

% wrapfigure

\begin{lemma}
Let $\AmmS \mid \confG[e]$ be a configuration, $\pmvA$ be an agent, $\valV[0]$ and $\valV[1]$ be natural numbers, $\tokT[0]$ and $\tokT[1]$ be tokens. If the following transition can be executed
%
\[
\AmmS \mid \confG[e]
    \xrightarrow{\actAmmSwap{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}}
    \AmmSi \mid
    \confG[e]' 
\]
\noindent
then the following equation holds 
%
\[
\fst(\AmmS.\ammF(\tokT[0], \tokT[1])) \times
\snd(\AmmS.\ammF(\tokT[0], \tokT[1]))
= 
\fst(\AmmSi.\ammF(\tokT[0], \tokT[1]) )\times
\snd(\AmmSi.\ammF(\tokT[0], \tokT[1]))
\]
\end{lemma}

\begin{lemma}
The execution of a $\ammSwapOp$ transaction from $\AmmS$ to $\AmmSi$ maintains the constant product constraint $(\ammR[0],\ammR[1]) = (\ammRi[0],\ammRi[1])$ for all $(\tokT[0], \tokT[1]) \in \dom(\AmmS.\ammM)$, where $(\ammR[0], \ammR[1])=\AmmS.\ammF(\tokT[0], \tokT[1])$ and $(\ammRi[0], \ammRi[1])=\AmmSi.\ammF(\tokT[0], \tokT[1])$.
\end{lemma}
\begin{proof}
Precondition $\circled{4}$ in eq. \ref{eq: amm swap transaction} can be written as $(\ammR[1]+\valV[1])\cdot(\ammR[0]+\valV[0]) = \ammR[0] \cdot \ammR[1]$ for $c_{fee}=0$. All other token pairs not involved in the swap remain unaffected by the swap transaction, and thus, the constant product invariant must hold there as well.
\end{proof}
\jamesnote{Proof is obvious, move to appendix}

\begin{lemma}
In a given AMM state $\AmmS$, where $\AmmS.\ammF(\tokT[0],\tokT[1]) > (0,0)$, the execution of a $\textsf{Swap}_{\pmvA}(\valV[0]:\tokT[0], \valV[1]:\tokT[1])$ is valid for finite unit amount of $\tokT[0]$ or $\tokT[1]$ transferable by $\pmvA$.
\end{lemma}
\jamesnote{For all funds such that rho (>0) there exists a transition ... (fresh is non-deterministic, system is determinstic up to renaming). Transferrable is not formal, should be balance of actor. Valid: For all v0 or v1.}

\jamesnote{Latex wrap figure for AMM graphs.}

\begin{proof}
Precondition \circled{1} of eq. \ref{eq: amm swap transaction} requiers a non-zero pair balance of $\tokT[0], \tokT[1]$. Precondition \circled{2} requires that the user $\pmvA$ performing the swap have a sufficient balance of tokens which it is transferring to the AMM. The constraint \circled{4} is solveable for any fixed, finite values of $\valV[0],\ammR[0], \ammR[1]$ or  $\valV[1],\ammR[0], \ammR[1]$. 
\end{proof}

\paragraph{AMM exchange rate properties:} Let us denote the exchange rate of a token pair $\tokT[0],\tokT[1]$ in AMM state $\AmmSi$ reachable from $\AmmS$ with a $\textsf{Swap}$ transaction as follows, where $\AmmS.\ammF(\tokT[0],\tokT[1]) > (0,0)$. 
\begin{equation} \label{eq: amm exchange rate}
    \textsf{exch}_{\AmmSi}(\tokT[0],\tokT[1]) = \parallel \frac{\partial}{\partial \ammRi[0]} \frac{\ammR[0] \cdot \ammR[1]}{\ammRi[0]} \parallel = \frac{\ammR[0] \cdot \ammR[1] }{(\ammR[0]^{\prime})^2} 
    \quad 
    \begin{array}{l}
        (\ammR[0], \ammR[1]) = \AmmS.\ammF(\tokT[0],\tokT[1]) \\
        \ammRi[0] = \fst(\AmmSi.\ammF(\tokT[0],\tokT[1])) \\
    \end{array}
\end{equation}
We write $\textsf{exch}_{\AmmSi}(\tokT[1],\tokT[0])$ as the inverse or equivalently as $\frac{\ammR[0]\cdot \ammR[1]}{(\ammRi[1])^2}$. However, we observe in precondition \circled{4} of the swap transaction rule (eq. \ref{eq: amm swap transaction}), that the exchange rate of $\valVi / \valV$ is dependent on the direction and magnitude of the swap. As such, we can define the \emph{effective} exchange rate as
\begin{equation}
    \begin{array}{l}
        \mathsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1]) = \frac{\ammR[1]}{\ammR[0]-\valV[0]} \quad
        \mathsf{effExch}_{\AmmS}(\valV[1]:\tokT[1],\tokT[0]) = \frac{\ammR[0]}{\ammR[1]-\valV[1]}
    \end{array}
\end{equation}
which denotes the ratio of token received over tokens transferred in a swap transaction. Here, the effective exchange rate $\mathsf{effExch}_{\AmmS}(\valV:\tokT,\tokTi)$ denotes the units in $\tokTi$ over $\tokT$, where a $\valV < 0$ denotes units transferred to the AMM and $\valV > 0$ units received. For a swap from $\tokT[0]$ to $\tokT[1]$ ($\valV[0]<0$), it can be observed that the effective price is lower than the exchange rate (eq. \ref{eq: amm exchange rate}) at the AMM state prior to the swap\footnote{In financial terms, this is referred to as slippage.}. 

\begin{lemma}
The exchange rate of an AMM pair $\textsf{exch}_{\AmmS}(\tokT[0],\tokT[1])$ will be reduced by a swap transaction from $\tokT[0]$ to $\tokT[1]$ ($\valV[0] < 0$), such that  $\textsf{exch}_{\AmmS}(\tokT[0],\tokT[1]) > \textsf{exch}_{\AmmSi}(\tokT[0],\tokT[1])$.
\end{lemma}
\begin{proof}
$\valV[0]< 0$ implies $\ammRi[0] > \ammR[0]$ in a swap transaction (eq. \ref{eq: amm swap transaction}). Therefore, by inspection of eq. \ref{eq: amm exchange rate}, $\textsf{exch}_{\AmmSi}(\tokT[0],\tokT[1])$ must be less than $\textsf{exch}_{\AmmS}(\tokT[0],\tokT[1])$ as $\ammR[0]\cdot\ammR[1]$ remains constant from $\AmmS$ to $\AmmSi$  (lemma 3) but $\ammRi[0] > \ammR[0]$. For brevity, we omit the proof for a swap in the opposite direction.
\end{proof}

\begin{lemma}
Transaction types $\ammDepositOp$ and $\ammRedeemOp$ applied to an AMM state $\AmmS$ where $\AmmS.\ammF(\tokT[0],\tokT[1]) > (0,0)$ do not affect the price of the token pair $\tokT[0],\tokT[1]$.
\end{lemma}

\begin{proof}
For a transaction $\actAmmDeposit{\pmvA}{\valV[0]}{\tokT[0]}{\valV[1]}{\tokT[1]}$ from $\confG$ to $\confGi$, the precondition \circled{1} of eq. \ref{eq: amm deposit transaction} implies $\valV[1] = \frac{\valV[0]}{\ammR[0]} \cdot \ammR[1]$. As such, we can observe that the price of the token pair remains constant:
\[
    \textsf{exch}_{\AmmSi}(\tokT[0],\tokT[1]) = \frac{(\ammR[0]+\valV[0])(\ammR[1]+\valV[1])}{(\ammR[0]+\valV[0])^{2}} =
    \frac{\frac{\ammR[1]}{\ammR[0]}\cdot(\ammR[0]+\valV[0])}{\ammR[0] + \valV[0]} = \frac{\ammR[1]}{\ammR[0]} =
    \textsf{exch}_{\AmmS}(\tokT[0],\tokT[1])
\]
Preconditions \circled{2}, \circled{3} in eq. \ref{eq: amm redeem transaction} imply $\valV[1] = \frac{\valV[0]}{\ammR[0]} \cdot \ammR[1]$ such that the price invariant must hold for $\actAmmRedeem{\pmvA}{\valV}{\tokT}$ as well.
\end{proof}

\subsection{Price Arbitrage}
The AMM provides incentives for users to interact with AMM pairs until the local pair price reflects the global average prices in $\exchO$: This incentive is denoted \emph{arbitrage} opportunity in financial terms, and is formalized in this section. If the effective exchange rates at an AMM differ from exchange rates implied by $\exchO$, and assuming a user can freely exchange tokens at the rate $\exchO(\tokT[0],\tokT[1])= \exchO(\tokT[1])/\exchO(\tokT[0])$, then a user can increase its token balance by executing a single swap transaction in our model. We illustrate this for the specific case $\exchO(\tokT[0],\tokT[1]) < \textsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1])$.

\begin{lemma}
If $\exchO(\tokT[0],\tokT[1]) < \textsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1])$ for a non-zero $\valV[0]$, a user with a non-zero balance of $\valV[0]$ can increase its balance of $\tokT[0]$ with a single swap transaction. \jamesnote{interaction with exch market outside model. Add tx rule for this swap.}
\jamesnote{Font: exch needs to be easily differentiated by font.}
\end{lemma}
\begin{proof} User $\pmvA$ with $\tokBal[\pmvA](\tokT[0]) \geq \valV[0]$ can freely swap $\valV[0]$ for units of $\tokT[1]$ at rate $\exchO(\tokT[0],\tokT[1])$, and subsequently swap these units of $\tokT[1]$ back to $\valVi[0]$ units of $\tokT[0]$ at the respective AMM pair $\tokT[0],\tokT[1]$, such that
\[
\valVi[0] = \mid \valV[0] \mid \cdot \frac{\exchO(\tokT[0],\tokT[1])}{\mathsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1])} > \valV[0]  
\] 
\end{proof}
Hence, an incentive for users to swap from $\tokT[1]$ to $\tokT[0]$ remains until  $\exchO(\tokT[0],\tokT[1])$ equals $\textsf{exch}_{\AmmS}(\tokT[0],\tokT[1])$: At this price equilibrium, $\exchO(\tokT[0],\tokT[1]) < \textsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1])$ cannot hold for a positive $\valV[0]$ and thus no arbitrage opportunity in this AMM token pair exists. We omit lemma and proof for the case $\exchO(\tokT[0],\tokT[1]) > \textsf{effExch}_{\AmmS}(\valV[0]:\tokT[0],\tokT[1])$. 

\subsection{Front-running}
Front-running assumes an adversary that has the ability to influence the ordering of transactions on the blockchain. For simplicity, we assume a single adversary $\pmvA$ that can order one transaction before and one following a given transaction performed by another user $\pmvB$. We consider the following trace, where adversary $\pmvA$ has ordered a swap transaction immediately before and after a swap transaction by $\pmvB$, where $(\valV[0], \valVi[0], \valV[1]) < (0,0,0)$. Note that $\pmvA$ simply swaps from $\tokT[0]:\tokT[0]$ to $\valV[1]:\tokT[1]$ \circled{1} and back \circled{3}. 
\begin{equation} \label{eq: amm front-running trace}
    \AmmS \xrightarrow{\circled{1}\;\mathsf{Swap}_{\pmvA}(\valV[0]:\tokT[0],\valV[1]:\tokT[1])}
    \AmmSi \xrightarrow{\circled{2}\;\mathsf{Swap}_{\pmvB}(\valVi[0]:\tokT[0],\valVi[1]:\tokT[1])}
    \AmmSii \xrightarrow{\circled{3}\;\mathsf{Swap}_{\pmvA}(\valVii[0]:\tokT[0],-\valV[1]:\tokT[1])} \AmmSiii
\end{equation}

\begin{lemma}
The execution of transaction trace in eq. \ref{eq: amm front-running trace} guarantees adversary $\pmvA$ an increased balance of $\tokT[0]$ or $\tokT[1]$ for $(\valV[0], \valVi[0], \valV[1]) < (0,0,0)$ or $(\valV[1], \valVi[1], \valV[0]) < (0,0,0)$ respectively.
\end{lemma}
\begin{proof}
For brevity, we provide a proof for case $(\valV[0], \valVi[0], \valV[1]) < (0,0,0)$. If swap transaction \circled{1} were followed directly by transaction \circled{3}, $\pmvA$ would receive an $\tokT[0]$ amount of $\valVii[0] = \frac{\ammR[1]}{\ammR[0] - \valV[0]}\cdot \frac{\ammR[0] - \valV[0]}{\ammR[1] + \valV[1] - \valV[1]} \cdot \valV[0] = \valV[0]$ (eq. \ref{eq: amm swap transaction}) from swap transaction \circled{3}, implying zero gain. However, if transaction \circled{3} is executed in the sequence in eq. \ref{eq: amm front-running trace}, we can observe that $\mathsf{effPrice}_{\AmmSi}(\valV[1]:\tokT[1], \tokT[0]) < \mathsf{effPrice}_{\AmmSii}(\valV[1]:\tokT[1], \tokT[0])$.
\[
\mathsf{effPrice_{\AmmSi}(\valV[1]:\tokT[1], \tokT[0])} = \frac{\ammR[0] + \valV[0]}{\ammR[1] - \valV[1] + \valV[1]} < \frac{\ammR[0] + \valV[0] + \valVi[0] }{\ammR[1] - \valV[1] - \valVi[1] + \valV[1]} = \mathsf{effExch}_{\AmmSii}(\valV[1]:\tokT[1], \tokT[0])
\]
This implies that $\valVii[0] > -\valV[0]$, which results in a gain for $\pmvA$ in $\tokT[0]$.
\end{proof}

% \begin{lemma}
% The \emph{effective price} of a $\mathsf{Swap}_{\pmvA}(\valV[0]:\tokT[0],\valV[1]:\tokT[1])$ transaction which results in a state transtion from $\AmmS$ to $\AmmSi$ is bounded by $\mathsf{price}_{\AmmS}(\tokT[0],\tokT[1])$ and $\mathsf{price}_{\AmmSi}(\tokT[0],\tokT[1])$ respectively.
% \end{lemma}
% \begin{proof}
% By inspection. For a $\valV[0] > 0$ the following must hold. For brevity, we omit the proof for $\valV[0] < 0$.
% \end{proof}

% \[
% \mathsf{price}_{\AmmS}(\tokT[0],\tokT[1]) = \frac{\ammR[1]}{\ammR[0]} < \mathsf{effExch}_{\AmmS}(\tokT[0],\tokT[1]) = \frac{\ammR[1]}{\ammR[0]+\valV[0]} < \mathsf{price}_{\AmmSi}(\tokT[0],\tokT[1]) = \frac{\ammR[1]-\valV[1]}{\ammR[0]+\valV[0]} 
% \]

==> basic_blockchain.tex <==
\section{A basic model of blockchains} 
\label{sec:basic-blockchain}

% \begin{table}[h]
%   \centering
%   \begin{tabular}{ll}
%     \hline
%     \begin{tabular}{ll}
%       $\pmvA,\pmvAi,\ldots \in \PmvU$ 
%       & users 
%       \\
%       $\tokT,\tokTi,\ldots \in \TokU$ 
%       & token types 
%       \\
%       $\tokBal \in \PmvU \rightharpoonup (\TokU \rightharpoonup \Nat)$
%       & user token balance \\
%       $\tokBal[\pmvA]$ 
%       & abbreviation of $\tokBal \pmvA$ 
%       \\
%     \end{tabular}
%       & \begin{tabular}{ll}
%           $\exchO \in \TokU[f] \rightarrow \Nat$ 
%           & price of free tokens
%           \\
%           $\confG, \confGi$ 
%           & blockchain state
%           \\
%           $\ell$ 
%           & action 
%           \\[-3pt]
%           $\confG\xrightarrow{\ell} \confGi$ 
%           & state transition
%         \end{tabular}
%     \\
%     \hline
%   \end{tabular}
%   \caption{Summary of notation.}
%   \label{table: notations - blockchain model}
% \end{table}

We start by introducing a basic model of blockchains, 
on top of which we will specify lending pools.
% \Cref{table: notations - blockchain model} 
% summarizes the notation used in the model. 
% The main components of our model are 
% \emph{tokens}, which represent crypto-assets,
% \emph{accounts}, which model users' balances, 
% and \emph{token prices}, which abstract price oracles.
% and \emph{blockchain rounds} (an abstraction of blocks or time).
% The basic blockchain model includes basic transactions to update token prices and blockchain rounds, which are later extended in the model of specific DeFi contracts.
We assume a set of \emph{users} $\PmvU$, ranged over by $\pmvA, \pmvAi, \ldots$,
and a set of \emph{token types} $\TokU$, ranged over by $\tokT,\tokTi,\ldots$.
We denote with $\TokU[f] \subseteq \TokU$ the subset of 
tokens types that can be freely transferred between users,
only assuming a sufficient balance of the sender
($\TokU[f]$ includes \eg the native blockchain tokens).
% , like bitcoins and ether).


\paragraph{Blockchain states} 

We model a blockchain state $\confG$ as a pair $\tokBal \mid \exchO$,
where $\tokBal \in \PmvU \rightharpoonup (\TokU \rightharpoonup \Nat)$
is a partial map representing the token balance of users,
and $\exchO \in \TokU[f] \rightarrow \Nat$
abstracts an oracle who prices the free tokens.
% and $\br \in \Nat^{+}$ is a blockchain round,
% representing the passing of time 
% (\eg, the blockheight in the Ethereum blockchain). 
% updated periodically, such as the blockheight in the Ethereum blockchain: It's update can be interpreted as the passing of a fixed time period.
Hereafter, we abbreviate $\tokBal \pmvA$ as $\tokBal[\pmvA]$. 
We use the standard notation $f \setenum{\bind{x}{v}}$ 
to update a partial map $f$ at point $x$:
namely, $f \setenum{\bind{x}{v}}(x) = v$, while
$f \setenum{\bind{x}{v}}(y) = f(y)$ for $y \neq x$.

Given a partial map $f \in \TokU \rightharpoonup \Nat$, a token type $\tokT \in \TokU$ and a partial binary operation  
$\circ : \Nat \times \Nat \rightharpoonup \Nat$, 
we define the partial map $f \circ \valV:\tokT$ as follows:
\begin{equation} \label{eq: balance update}
  f \circ \valV:\tokT = \begin{cases}
    f\setenum{\bind{\tokT}{f(\tokT) \;\circ\; \valV}}
    & \text{if $\tokT \in \dom{f}$ and $f(\tokT) \circ \valV$ is defined} \\
    %f\setenum{\bind{\tokT}{0}} & \text{if $\tokT \in \dom{f}$ and $\valVi \circ \valV$ is undefined} 
    %\\
    f\setenum{\bind{\tokT}{\valV}}
    & \text{if $\tokT \not\in \dom{f}$}
  \end{cases}
\end{equation}

\noindent
% For instance, 
We adopt the notation $\valV:\tokT$ to denote $\valV$ units of token $\tokT$ throughout the paper.


\paragraph{State transitions} 

We model the interaction between users and the blockchain 
as a state transition system,
with labels $\ell$ which represent transactions and
updates of the price oracle.
Our basic model has only one kind of transaction,
denoted by $\actTransfer{\pmvA}{\pmvB}{\valV:\tokT}$,
which models the transfer of $\valV$ units of token $\tokT$ 
from user $\pmvA$ to user $\pmvB$. 
Its effect on the blockchain is modelled by the following rule:

\begin{equation*} 
  \label{eq:Trf}
  \irule
  {\begin{array}{cccc}
     \circled{1}\; \tokBal[\pmvA](\tokT) \geq \valV \quad\;
     & \circled{2}\; \tokT \in \TokU[f] \quad\;
     & \circled{3}\; \tokBali[\pmvA] = \tokBal[\pmvA] - \valV:\tokT \quad\;
     & \circled{4}\; \tokBali[\pmvB] = \tokBal[\pmvB] + \valV:\tokT
   \end{array}}
 {
   \tokBal \mid \exchO
   \xrightarrow{\actTransfer{\pmvA}{\pmvB}{\valV:\tokT}}
   \tokBal \setenum{\bind{\pmvA}{\tokBali[\pmvA]}} \setenum{\bind{\pmvB}{\tokBali[\pmvB]}} 
   \mid \exchO 
 }
 \;\nrule{[Trf]}
\end{equation*}
We decorate rule preconditions with circled numbers, \eg \circled{1}, 
to simplify their reference in the text. 
Rule \nrule{[Trf]} states that the transfer is permitted whenever
the sender has a sufficient balance \circled{1}, 
and the transferred token type is free \circled{2}.

The following rule models the non-deterministic update of the price oracle:
\begin{equation*} 
  \label{eq: token price update}
  \irule{}
  {
    \tokBal \mid \exchO
    \xrightarrow{\exchUpdateOp} 
    \tokBal \mid \exchOi
  }
  \;\nrule{[Px]}
\end{equation*}



\endinput

Note that DeFi contract types which implement interest rates will require the periodic \emph{compounding} of interest (\S \ref{section: financial terms}): We update the blockchain round update transaction $\xrightarrow{1}$ rule later when such DeFi archetypes are introduced to our model. 
\jamesnote{WIP: Remove rounds, note the reasoning here.}


==> ext_model.tex <==
\section{DeFi Vulnerabilities}

\subsection{Extended Blockchain Model}
\jamesnote{WIP: Authorization predicates introduced to protect user against adversarial scheduling of authorized transactions.}


\paragraph{Blockchain Interaction:} 
We model the system state of users appending transactions to the blockchain as the tuple $(\confG, K)$, where $K$ denotes the shared knowledge of users on the blockchain network. In order for a transaction to be appended to the blockchain, its authorization must first be \emph{announced} on the network. For brevity, we write $\authTx$ for $\authTx(\tn[\pmvA](\appFuncArgs))$.

\begin{equation} \label{eq: Transaction Authorization}
\irule 
    {} %Empty 
    {
        (\confG, K) \xrightarrow{\authTx} (\confG, K \cup \left\{ \authTx \right\})
    }
\end{equation}
Transactions with known, valid authorizations can be appended to the blockchain. 
\begin{equation} \label{eq: Transaction Execution}
\irule
    {
        \confG \xrightarrow{\tn[\pmvA](\appFuncArgs)} \confGi \quad
        \authTx \models \tn[\pmvA](\appFuncArgs), \confG \quad
        \authTx \in K
    } %Empty 
    {
        (\confG, K) \xrightarrow{\tn[\pmvA](\appFuncArgs)} (\confGi, K)
    }
\end{equation}

\noindent
\jamesnote{A user can authorize a transaction, but not schedule their execution.}

We now introduce our model of lending pools and extend our blockchain model with additional transaction types describing the interaction of user accounts with lending pool instances.


\subsubsection{Authorizations}
For a transaction $\tn[\pmvA]$ to be appended to a blockchain state $\confG$, $\pmvA$ must provide an authorization $\authTx(\tn[\pmvA](\appFuncArgs))$: This authorizes the transaction $\tn[\pmvA](\appFuncArgs)$ to be applied to any blockchain state $\confG$. 

We write that $\authTx \models \tn, \confG$ holds, if $\authTx = \authTx(\tn[\pmvA](\appFuncArgs))$ and $\tn = \tn[\pmvA](\appFuncArgs)$ and it can be executed in $\confG$. \\
\albertonote{in the rule below we use auth without arguments} \\
\jamesnote{@AL: See changes} \\ 
\albertonote{this executability condition is left underspecified, correct?} \\
\jamesnote{@AL: Do you mean eq. 5?}

\subsubsection{Authorization w/ Predicates}   
\jamesnote{Postpone to section 3.}
Given our blockchain model which includes lending pools and exchange rates for token types, we also extend a transaction authorization $\authTx(\tn[\pmvA](\appFuncArgs), \authPr)$ to include a predicate $\authPr$ on the blockchain configuration $\confG$: This authorizes the transaction $\tn[\pmvA](\appFuncArgs)$ to be applied to any blockchain state $\confG$, which fulfills the predicate $\authPr \in \mathbb{\Gamma} \rightarrow bool$. We write that $\authTx(\tn[\pmvA](\appFuncArgs), \authPr) \models \tn, \confG$ holds, if $\tn = \tn[\pmvA](\appFuncArgs)$ and the authorization enables the $\tn$ to be appended to blockchain state $\confG$. 

This need for authorization predicates arises from the fact that user accounts can \emph{authorize} transactions, but cannot \emph{schedule} these on the blockchain: The utility of a user-authorized transaction is \emph{predicated} on the blockchain state the transaction is applied to. For a rational agent, this utility is a function of token exchange rates and lending pool state. For example, a user's decision to liquidate a loan is made based on exchange rates $exch$, which may change between the authorization and execution of the transaction.

\subsubsection{Atomic Transaction Groups}
A user account can authorize a transaction \emph{sequence} $\tnA[\pmvA] = \tn[\pmvA, 1], \cdots, \tn[\pmvA, n]$ to execute from a specified blockchain state $\confG$, such that the following holds for some $\confG[1] \cdots \confG[n]$
\[
    \confG \xrightarrow{\tnA[\pmvA](\appFuncArgsA)} \confG[n] = 
    \confG \xrightarrow{\tn[\pmvA,1](\appFuncArgs[1])} \confG[1]
    \cdots \confG[n-1]
    \xrightarrow{\tn[\pmvA, n](\appFuncArgs[n])} 
    \confG[n]
\]
where $\appFuncArgsA = \appFuncArgs[1], \cdots , \appFuncArgs[n]$. We denote the intermediary states $\confG[1] \cdots \confG[n-1]$ as \emph{sub-states} and $\confG, \confG[n]$ as \emph{full-states}. We now extend a user transaction authorization to $\authTx(\tnA[\pmvA](\appFuncArgsA), \authPr)$ which authorizes the \emph{sequence} of transactions to be applied to a blockchain configuration $\confG$ where $\authPr(\confG)$ holds true. Since such an authorization does not authorize the transactions in the sequence to execute individually or an alternative order, it's execution is necessarily atomic. For transaction sequences with $|\tnA| \geq 1$ we now replace our previous transaction execution rule (\ref{eq: Transaction Execution}) for atomic transaction sequences.
\begin{equation}
\irule
    {
        \confG \xrightarrow{\tnA} \confGi \quad
        \authTx \models \tnA, \confG \quad
        \authTx \in K
    } %Empty 
    {
        (\confG, K) \xrightarrow{\tnA} (\confGi, K)
    }
\end{equation}


\subsection{Extractable Value from Liquidations:} For a lending pool with non-empty set of liquidatable accounts, a rational actor's strategy will be to authorize the liquidation of all accounts, such that the risk-free profit it can extract from the lending pool is maximized, and no "profit opportunity" remains.

In particular, we assume the rational actor has a preference for collateral token types which can be immediately redeemed from the lending pool for the underlying token type $\uTok(\tokT)$ where $\tokT \in \minted(\LpS)$. As such, the rational agent's liquidation strategy of a lending pool is given by
\begin{itemize}
    \item $L \in \PmvU \rightarrow (\TokU \times \TokU \rightarrow \Nat)$ is a liquidation of a lending pool
\end{itemize}
where the co-domain $(\TokU \times \TokU \rightarrow \Nat)$ is a map from repaid and seized collateral ($\TokU \times \TokU$) token types to seized collateral units ($\Nat$), which are immediately withdrawn from the lending pool. The optimal liquidation strategy $L$ is determined by 
\begin{equation}
    \argmax_{L} \sum_{\pmvA \in \dom(L)} \sum_{(\tokT, \tokTi) \in \dom(L(\pmvA))}
    \frac{L(\pmvA, (\tokT, \tokTi))}{\exchO(\uTok(\tokTi))}
\end{equation}
Subject to constraints
\begin{itemize}
    \item $\dom(L) \subseteq liqAcc_{\LpS}$
    % \item $\TokU_{repay} \subseteq \bigcup_{\pmvA \in \PmvU_{liq}} \borrTok[\LpS](\pmvA)$
    % \item $\TokU_{coll} \subseteq \bigcup_{\pmvA \in \PmvU_{liq}} \collTok[\LpS](\pmvA)$
    \item $\forall \pmvA \in \dom(L):$
    \begin{itemize}
        \item $sCollVal_{\LpS}(\pmvA) \geq \sum_{(\tokT, \tokTi) \in \dom(L(\pmvA))}
    \frac{L(\pmvA, (\tokT, \tokTi))}{\exchO(\uTok(\tokTi))}$ 
        \item $\forall \tokT \in \fst(\dom(L(\pmvA))) :
            \frac{\LpS.\lpB(\pmvA, \tokT)}{\exchO(\tokT)} \geq 
                \sum_{\tokTi \in \snd(\dom(L(\pmvA)))} \frac{L(\pmvA, (\tokT, \tokTi))}{\exchO(\tokTi) \cdot r_{liq}}$
        \item $\forall \tokTi \in \snd(\dom(L(\pmvA))) :
            \tokBal[\pmvA](\tokTi) \geq 
                \sum_{\tokT \in \fst(\dom(L(\pmvA)))} L(\pmvA, (\tokT, \tokTi))$
    \end{itemize}
    \item $\forall \tokTi \in \minted(\LpS) :$
    \begin{itemize}
        \item $\LpS.\lpF(\uTok(\tokTi)) \geq \sum_{\pmvA \in \dom(L)} 
    \sum_{\tokT \in \fst(\dom(L(\pmvA)))} L(\pmvA, (\tokT, \tokTi))$
    \end{itemize}
\end{itemize}



\subsection{Flash-Loans}

Lending pools implement flash loans which must be repaid within a single atomic transactions sequence. For token types $\tokT \notin \minted(\LpS)$, transaction types $\sborrowOp$ and $\srepayOp$ defined as
\begin{equation}
\irule
{\begin{array}{l}
    \LpS.\lpF(\tokT) \geq \valV > 0 \qquad
    \lpFfuni = \LpS.\lpF - \valV:\tokT \qquad
    \tokT \notin \minted(\LpS)
\end{array}}
{
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid \LpS \mid 
    \confG[e]
    \xrightarrow{\actSborrow{\pmvA}{\valV:\tokT}}
    \confDep{\pmvA}{\tokBal[\pmvA] + \valV:\tokT} \mid
    \LpS \setenum{ \lpF = \lpFfuni}  \mid
    \confG[e] 
}
\; \nrule{[fBorrow]}
\end{equation}

\begin{equation}
\irule
{\begin{array}{l}
    \tokBal[\pmvA] \geq \valV > 0 \qquad
    \lpFfuni = \LpS.\lpF + \valV:\tokT \qquad
    \tokT \notin \minted(\LpS)
\end{array}}
{
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid \LpS \mid 
    \confG[e] 
    \xrightarrow{\actSrepay{\pmvA}{\valV:\tokT}}
    \confDep{\pmvA}{\tokBal[\pmvA] - \valV:\tokT} \mid
    \LpS \setenum{ \lpF = \lpFfuni}  \mid
    \confG[e]
}
\; \nrule{[fRepay]}
\end{equation}

For each $\sborrowOp(\pmvA, \valV:\tokT)$ function execution along an atomic group sequence, a subsequent $\srepayOp(\pmvA, \valVi:\tokT)$ execution must follow in the same atomic group, such that $\valVi - \valV \geq \exchO(\tokT) \cdot C_{fee}$. \jamesnote{WIP: How to describe this more formally in temporal logic?} \\


\noindent
Our lending pool model also implements transaction types to offer flash loan for minted tokens: Here, no maximum loan amount threshold exists. Each $\sborrowMOp(\pmvA, \valV:\tokT)$ along an atomic group sequence must be followed by a $\srepayMOp(\pmvA, \valV:\tokT)$ transaction, where $\valV = \valVi$: The fee is paid in a token type not minted by the lending pool.
\begin{equation}
\irule
{\begin{array}{l}
    \valV > 0\qquad
    \tokT.\tokOwn = \LpS \qquad
    \lpMfuni = \LpS.\lpM + \valV:\tokT  \qquad
    \tokT \in \minted(\LpS)
\end{array}}
{
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid \LpS \mid 
    \confG[e] \mid
    \br
    \xrightarrow{\actSborrowM{\pmvA}{\valV:\tokT}}
    \confDep{\pmvA}{\tokBal[\pmvA] + \valV:\tokT} \mid
    \LpS \setenum{ \lpM = \lpMfuni}  \mid
    \confG[e] \mid
    \br
}
\nrule{[fBorrowM]}
\end{equation}


\begin{equation}
\irule
{\begin{array}{l}
    \tokBal[\pmvA](\tokT) \geq \valV > 0 \qquad
    \tokBal[\pmvA](\tokTi) \geq \valVi > C_{fee} \cdot \exchO(\tokTi) \qquad
    \\[5pt]
    \tokT \in \minted(\LpS) \qquad
    \tokTi \notin \minted(\LpS) \qquad
    \lpMfuni = \LpS.\lpM - \valV:\tokT \qquad
\end{array}}
{
    \confDep{\pmvA}{\tokBal[\pmvA]} \mid \LpS \mid 
    \confG[e] \mid
    \br
    \xrightarrow{\actSrepayM{\pmvA}{\valV:\tokT, \valVi:\tokTi}}
    \confDep{\pmvA}{\tokBal[\pmvA] - \valV:\tokT} \mid
    \LpS \setenum{ \lpM = \lpMfuni}  \mid
    \confG[e] \mid
    \br
}
\nrule{[fRepayM]}
\end{equation}



\subsection{On-chain Exchange Rates}

We now extend our lending pool model to obtain exchange rates from on-chain automatic market makers. We sketch an automatic market maker as a stateful object in the blockchain configuration which can be updated by a transaction authorizable by a user, who performs a trade.
\begin{equation}
\irule
{}
{
    M \mid
    \confG[e] 
    \xrightarrow{trade_{\pmvA}} 
    M' \mid
    \confG[e]  
}
\end{equation}
The function $rate_{M} \in \tokT \rightarrow \mathbb{R}^+$ returns the token price based on the current state of the automatic market maker $M$. We can update the account collateralization (eq. \ref{eq: Account Collateralization}) to be computed from the automatic market maker state $M$.
\begin{equation} \label{eq: Account Collateralization w/ AMM}
\Coll{\LpS}{\confDep{\pmvA}{\tokBal}}{M} = \dfrac
{\sum_{\tokT \in \collTok[\LpS](\pmvA)} rate_{M}(\uTok(\tokT))\cdot\ER[\LpS]{\uTok(\tokT)} \cdot \tokBal(\tokT)}
{\sum_{\tokT \in \borrTok[\LpS](\pmvA)} rate_{M}(\tokT) \cdot \LpS.\lpB(\pmvA,\tokT)}
\end{equation}

\paragraph{Market Equilibrium Assumption:} In order for the borrowed funds of the lending pool to be properly secured, it is important that the collateralization is computed with exchange rates at which a user trade can actually perform asset exchanges: $rate_{M}$ must reflect \emph{market rates}. Assuming $\exchO$ provides global market rates, a state $\confG = \langle M \mid \exchO \mid \confG[e] \rangle$ in which the set $arb(\confG) = \left\{\tokT \mid \exists \tokT : |rate_{M}(\tokT) - \exchO(\tokT)| > 0 \right\}$ is non-empty, we assume with overwhelming high probability that subsequently executed transaction (group) $\tnA_{\pmvA}$ results in a state $\confGi = \langle M' \mid \exchO \mid \confG[e] \rangle$, where set $arb(\confGi)$ is empty: The possible arbitrage trades in $M$ have been taken by $\pmvA$. Assuming flashloans are widely available for all token types, such an actor needn't even require an upfront balance of relevant tokens.

However, the market equilibrium assumption cannot hold in a \emph{sub-state} during the execution of an atomic transaction group $\tnA[\pmvA]$. Since a single user controls the transaction sequence, it can manipulate the state of $M$ arbitrarily in sub-states of $\tnA[\pmvA]$: For example, an initial trade by a user in an atomic transaction group resulting in an automatic market maker state $M'$, where $rate_{M'}(\tokT) \neq \exchO(\tokT)$, may allow the discounted liquidation of accounts, which would be sufficiently collateralized at exchange rates in $\exchO(\tokT)$. This user can subsequently perform a trade in the opposite direction within the same atomic transaction group, such that $arb(\confGi)$ is empty upon completion of the atomic group. This illustrates that market prices cannot be assumed in \emph{sub-states} during the execution of an atomic transaction group.

In order for the collateralization of an account to be computed based on \emph{market exchange rates}, the lending pool must have access to the last prior \emph{full-state}, where the market equilibrium assumption can hold for contracts such as automatic market makers. \jamesnote{WIP: I am unsure how market equilibrium assumption is affected in presence of "miner extractable value".}

\subsection{Most Recent Full-State}
We denote $L(\confGi)$ as the most recent \emph{full-state} as seen from state $\confGi$. If $\confGi$ is a full-state, then  $L(\confGi) =  \confGi$. For brevity, we adopt this notation for fragments of a configuration. For a atomic transaction group 
\[
    \tnA[\pmvA] = 
    \langle \LpS \mid M \mid \confG[e] \rangle 
    \xrightarrow{\tn[\pmvA,1]}
    \langle \LpS[1] \mid M_{1} \mid \confG[e] \rangle
    \cdots
    \langle \LpS[n-1] \mid M_{n-1} \mid \confG[e] \rangle
    \xrightarrow{\tn[\pmvA, n]} 
    \langle \LpS[n] \mid M_{n} \mid \confG[e] \rangle
\]
$L(M_{i})$ evaluates to $M$ for all $i \neq n$ and to $M_{n}$ for $i=n$. We now update equation \ref{eq: Account Collateralization w/ AMM} by replacing $rate_{M}$ with $rate_{L(M)}$, such that asset exchange rates are determined from the last full-state of an on-chain automatic market maker.
